Synthetic chest radiographs with dense anatomical segmentation masks derived from computed tomography

Pixel-level anatomical annotation of chest radiographs is laborious and inter-reader agreement is limited, constraining the development of dense segmentation models. We present PAXRay++, a collection of synthetic chest radiographs derived from computed tomography (CT) by a deterministic projection pipeline. It contains 14,374 two-dimensional frontal and lateral projections, each paired with pixel-level masks for 159 anatomical classes, totalling more than 1.6 million labeled instances. Masks were produced by ensembling three-dimensional CT segmentation models, applying rule-based anatomical post-processing, and projecting the labels onto the synthetic radiographs. Annotation quality was assessed through automated consistency checks and an expert correction experiment on independent real radiographs, where agreement was high for large structures and lower for thin or superimposed ones. The resource supports the development and evaluation of fine-grained anatomical segmentation in chest radiographs.

==> sections/results_subfiles/dataset_generation.tex <==
\input{figures/dataset_stats}

==> sections/results_subfiles/test_performance.tex <==
\input{figures/test_qual}

==> sections/results_subfiles/validation_performance.tex <==
\input{figures/validation_qual}

==> sections/text_storage.tex <==

\iffalse 



% Chapter X

% \chapter[Learning from Partially Annotated  Domains]{Learning from Partially \newline  Annotated  Domains} % Chapter title

\label{ch:partial_domains} % For referencing the chapter elsewhere, use \autoref{ch:name} 

%----------------------------------------------------------------------------------------


% % \begin{mdframed}[hidealllines=true,backgroundcolor=gray!20]

A medical report has to convey  a vast range of information to cover the any state of visible organs. However, most medical datasets focus strictly on a specific set findings or organs, but do not consider their surroundings. In this chapter, we aim to unify the available information to provide necessary context to different imaging domains.
We start by paving the way for CT to X-Ray translation and show how we can make use of a variety of partial labels from the CT domain to segment anatomy of X-Rays in Section~\ref{sec:ch5_bmvc_dataset}. Afterwards, we expand on this prove of concept and display ways to scale this data collection process through self-training in Section~\ref{sec:ch5_nature}. Finally, in Section~\ref{sec:ch5_bmvc_grounding}, we make the connection between vision and language as we ground reported findings in X-Rays via their associated anatomical descriptions.
% \end{mdframed}

% % \input{Chapters/05_learningfrompartialdata/figures/dataset/dataset_creation.tex}

While the incorporation of unlabeled data can heavily benefit the training of deep learning models, one still has to acquire enough data to kickstart the process. For our goal of achieving a holistic understanding of a given image, this can pose as quite troublesome since we have to gather annotations for a vast variety of labels. For segmentations in X-rays, this issue is exacerbated due to the body absorbing radiation to a highly varying degree leading to anatomical structures in two-dimensional images being visibly overlayed with each other.
As the complete anatomic annotation for a single image already took up to three hours due to the ambiguity of overlapping structures~\cite{seibold2022reference}, an entire dataset appears as a daydream. 

Is there any way we can gather the required labels without hiring an army of medical staff for annotation purposes?  We take a look at other radiology subdomains and notice most datasets focus on a specific subset relevant to their specialty, i.e. segmentations of Thoracic Organs at Risk~\cite{lambert2020segthor} or the spine~\cite{sekuboyina2021verse} in CT volumes. These datasets partially comprising of less than a 100 patients have shown to enable the development of robust networks transferrable to new data~\cite{isensee2021nnu}. We assume that by aggregating all these different annotations, we can achieve a rather complete outlook on the human body. 

Assuming this is achievable, we now face one final obstacle in order to utilize these annotations for our CXR report generation models: As most considered datasets are in the CT domain, we have to find way to translate this information to CXRs. While this task of domain adaptation is typically difficult, we make use of the fact that the CT albeit being a volumetric imaging modality directly build upon the two-dimensional X-Ray. Therefore, as these modalities share several visual features, we can formulate a back-projection to map not only the CT but also the associated annotations to a two-dimensional plane, simulating an X-Ray.

The following sections build upon the idea of utilizing the CT domain to aggregate various annotations and, by using the corresponding projections, enable the accurate segmentation of chest radiographs.



\section{Annotations of Chest X-Rays via Computer Tomography Projection}\label{sec:ch5_bmvc_dataset}
The following section is based on our publication in \textit{BMVC 2022}~\cite{Seibold_2022_BMVC}.\\
% \input{Chapters/05_learningfrompartialdata/05_01_paxrayv1.tex}
\section{Extending the PAXRay dataset}\label{sec:ch5_nature}
% \input{Chapters/05_learningfrompartialdata/05_03_expandingpaxray.tex}
\newpage
\section{Grounding Medical Reports via Anatomy Descriptors}\label{sec:ch5_bmvc_grounding}
% \input{Chapters/05_learningfrompartialdata/05_04_grounding}
% % \input{Chapters/05_learningfrompartialdata/05_02_diffusion.tex}

\section{Chapter Conclusion}

In this chapter, we follow the idea that we can leverage anatomical annotations from various sources in a pixel-wise distinct CT-domain to develop segmentation models in the difficult to annotate X-Ray domain. We build on the shared underlying source of radiation, which allows to construct a projection from a CT volume that resembles a common X-Ray. This allows us to aggregate a vast variety of anatomical labels in CT domain and then project these with the volume to a two dimensional plane to simulate X-ray training data. 

We first show in a small scale experiment that this setup can to produce anatomy segmentation models. These can, in turn, be used to ground anatomical information from medical reports. We have shown, that such anatomical segmentations can serve as better region proposals for the grounding of medical phrases than common proposal methods. 

After establishing the validity of this approach, we scaled up the PAX-Ray dataset by integrating more relevant labels as well as using more thorax CT's as a basis for translation. We merge labels from ten sources on a seperate dataset via a set of rules and label post-processing. After training on this joint label set, we run inference on six sufficiently large thorax ct datasets to in the end gather more than 7000 pseudolabeled CTs. Training on the projections of these volumes presented us with segmentation models that have a high agreement with medical personal on real CXR data.


We summarize our contributions as:


% \begin{mdframed}[hidealllines=true,backgroundcolor=gray!20]
 \textbf{Contribution 1:} We show how we can utilize existing CT annotations for the analysis of CXR. By merging annotations of multiple partially annotated datasets and projecting these onto a two dimensional plane we can effectivly train deep learning based models. This allows us to build the first robust anatomy segmentation model for CXR.
% \end{mdframed}

% \begin{mdframed}[hidealllines=true,backgroundcolor=gray!20]
 \textbf{Contribution 2:} We build the PAX-Ray++ dataset, the first dataset with dense anatomical annotations in the CXR domain spanning label categories from abdominal and mediastinal regions to specific bones and organs. This datasets contains more than 14.000 images and is with more than 2 million instances comparable to real world datasets such as MS COCO. 
% \end{mdframed}

% \begin{mdframed}[hidealllines=true,backgroundcolor=gray!20]
 \textbf{Contribution 3:} We show the use of anatomical segmentations by applying them to the task of medical phrase grounding. While common region proposal mechanisms fail on this medical domain, anatomical segmentations provide a better anchor for vision-language understanding.
% \end{mdframed}


While our approach has enabled the first holistic segmentation of the human anatomy in CXR without the need of \textit{any} manual annotation in that domain, we have to note potential shortcomings. CTs are typically a much scarcer resource than the common CXR making it difficult to scale this approach to the levels of natural image datasets with millions of images due the overall lack of volumetric data. CXR also tend to use a slightly harder type of radiation compared to standard CTs. This fact paired with the common use of contrast agents in CTs might lead to a divergence of visual quality between the projected X-rays and real ones.  
We, however, believe that this can be salvaged through a more sophisticated use of backprojection either via physical simulations or generative models.



 As we have shown, most datasets in the CXR domain rely on either automatically parsed pathology labels or complete medical reports.
While this has rapidly advanced the field of automated X-Ray processing, dense masks, which are essential in many computer vision approaches, have taken a backseat due to the immense difficulty of gathering precise annotations for such overlapping structures. 
As CTs allow for easier recognition of specific structures due to their volumetric characteristic, we propose a new method for generating annotations for X-Rays using them to address this challenge. Our approach, which we illustrate in Fig.~\ref{fig:dataset_creation}, involves collecting annotations from existing CT models, projecting them onto 2D images that mimic the X-Ray domain, and creating a finely labeled dataset for anatomy segmentation in both frontal and lateral views. Using the shared imaging basis, we leverage the similarities in anatomy between different imaging modalities.



\subsection{Automated Generation of Projected CXR Datasets} 
In previous chapters, we built deep learning models to recognize anatomies or findings on the X-Ray domain in an end-to-end manner without considering the mechanics underlying the imaging process. This narrows our understanding of potential connections to other imaging modalities. Therefore, we will first examine the similarities and differences between CT and X-Ray imaging and then demonstrate how we can use this information to create accurately labeled datasets.




% \input{Chapters/05_learningfrompartialdata/figures/dataset/label_overview.tex}
\quad

\subsubsection{Automated Label Generation}\label{sec:label_mapping}

The emergence of the UNet has significantly improved the accuracy of 3D medical image segmentation~\cite{unet,cciccek20163d,isensee2021nnu}. In our annotation process, we use both proven traditional methods~\cite{lassen2011lung, lassen2012automatic} and the state-of-the-art nnUNet~\cite{isensee2021nnu}, which has shown great potential as a black-box segmentation model.
% \input{Chapters/05_learningfrompartialdata/figures/dataset/dataset_example.tex}


Our annotation scheme is based on a label hierarchy with each label mask represented by $\mathcal{M}_{l}$, where $l \in L$ and $L$ is the set of considered labels. We begin by generating a body mask $\mathcal{M}_{body}$ to separate it from the CT-detector backplate by selecting the largest connected component after thresholding as described previously. We then consider the super-categories of ~\textit{bones}, ~\textit{lung}, ~\textit{mediastinum} and ~\textit{sub-diaphragm}. In general, we assume that each fine-grained class is a subset of its parent class, such as the spine within the bone structure ($\mathcal{M}_{spine} \subset {M}_{bone}$). We obtain $\mathcal{M}_{bone}$ through slicewise generalized histogram thresholding~\cite{barron2020generalization}. Within the bone structure, we segment the individual vertebrae using a nnUNet~\cite{isensee2021nnu} trained on the Verse dataset~\cite{loffler2020vertebral,sekuboyina2021verse,liebl2021computed} and on ribs from RibFrac~\cite{yang2021ribseg}.
For Verse, the final validation performance ranges between 0.82 and 0.84 across all splits. We extend the rib annotation of Yang~\etal\cite{yang2021ribseg} by distinguishing individual ribs as well as posterior and anterior parts based on their center and horizontal inflection. 

For the lungs, we use the lung lobe segmentation model by Hofmanninger~\etal~\cite{hofmanninger2020automatic}. The reported dice score for their lung segmentation model of 0.99, 0.94, and 0.98 on the LTRC~\cite{ltrc}, LCTSC~\cite{yang2017data}, and  VESS12~\cite{rudyanto2014comparing} datasets respectively.
The merger of the individual lobes results in the lung halves. We further obtain the pulmonary vessels and total lungs through calculated thresholding and post-processing strategies~\cite{lassen2011lung}.


For the mediastinum, we consider the area between the lung halves. To segment this area, we utilize Koitka~\etal's Body Composition Analysis (BCA)\cite{koitka2021fully} and split it into superior and inferior along the 4th T-spine following medical definitions\cite{cook2015anatomy}. 
 Koitka~\etal~\cite{koitka2021fully} show a performance for their BCA of 0.96 dice on their internal dataset. We extract annotations for the \textit{heart}, \textit{aorta}, \textit{airways}, and \textit{esophagus} using the SegThor dataset~\cite{lambert2020segthor}.
The final validation performance for the nnUNet trained on SegThor ranges between 0.91 and 0.93 across all splits. 

As for the sub-diaphragm, we consider the area below the diaphragm. This area can be extracted from the soft tissue region segmented using the BCA, which we split centrally into the left and right hemidiaphragm as there is no anatomical indicator.

To generate the label set $L$, we apply the combination of mentioned networks and rulesets on the publicly available RibFrac~\cite{ribfrac2020} dataset, which is suitable for this projection process due to its focus on the thoracic area, the high axial resolution, and the scans being recorded without contrast agents similar to X-Rays. We ignore volumes with conflicting segmentations and manually remove volumes with noticeable errors.

We project these labels to 2D using the $\max$ operation along the desired dimension and apply post-processing steps based on the observed anatomy (i.e., restricting specific classes to their largest connected component). Doing so, lets us collect the \textbf{P}rojected \textbf{A}natomy for \textbf{X-Ray} dataset (PAX-Ray) consisting of 852 images with associated masks.

\subsubsection{Further Visual Examples of Generated Labels}
% \input{Chapters/05_learningfrompartialdata/figures/supplementary/3dsuppslice.tex}
We show examples of the annotations of our dataset in Fig.~\ref{fig:paxray_examples}. We can see that lung halves can overlap in the second frontal row. While this might seem contradictory at first, when considering the lung as a 3D volume, the classes can overlap along one dimension, i.e., the lung halves in front and behind the heart, as seen in Fig.~\ref{fig:3dslice_supp}. As we intend to capture the entire anatomy of the upper body, we consider this labeling assumption a more holistic approach. 
% \input{Chapters/05_learningfrompartialdata/figures/supplementary/dataset.tex}
\subsection{Experimental Setup}\label{sec:eval_segmentation}
% In this subsection, we first evaluate the different factors for segmentation quality such as architecture and initialization on our dataset in Sec.~\ref{sec:eval_segmentation}.  We, hereby, show the qualitative effect of PAXRay pre-trained models on real and projected chest X-Rays. 
% Afterwards, we highlight the usability of our anatomy segmentations for other tasks with the example of medical phrase grounding in Sec.~\ref{sec:eval_grounding}.
% \input{Chapters/05_learningfrompartialdata/figures/experiments/qualitative_results_segmentation_paxray.tex}
% \input{Chapters/05_learningfrompartialdata/figures/experiments/qualitative_results_segmentation.tex}



% \begin{landscape}
\begin{figure}[!p]
   \centering
    %\includegraphics[width=1.0\textwidth]{Image.eps}
    \includegraphics[height=0.41\textheight,angle=270]{Chapters/05_learningfrompartialdata/figures/_images/bmvc/plot.png}
    \caption{Segmentation performance in IoU on the test split for all classes of our proposed PAXRay dataset}
    \label{fig:bmvc_iou_all_clases}
\end{figure}
% \end{landscape}

% \input{Chapters/05_learningfrompartialdata/tables/bmvc/experiments/segmentation_results.tex}

\noindent{\textbf{Evaluation Setup:}} 
To assess the accuracy of our segmentation method, we utilize the mean Intersubsection over Union (IoU) measure on the PAXRay dataset. We follow the train/val/test split established in the RibFrac dataset~\cite{ribfrac2020}, resulting in a total of 598, 74, and 180 images in the train, validation, and test sets, respectively. During the training process, we evaluate the performance of our model on the validation set every 10 epochs and ultimately choose the model that performs best on the validation set for our final test.

\noindent\textbf{Implementation Details:}
To demonstrate the effectiveness of our fine-grained multi-label dataset, we trained segmentation models using different backbone networks, including the UNet (commonly used in the medical field) and the SFPN with a ResNet-50 backbone. We also compare the use of pre-training on the VinBigDataset~\cite{nguyen2020vindr} with using the networks from scratch. Since the labels may overlap, we used binary cross-entropy and a binary dice loss during training. We also employed random resize-and-cropping (with a range of $[0.8, 1.2]$) as an augmentation technique. We used AdamW optimization with a learning rate of 0.001 for 110 epochs, decaying by a factor of 10 at epochs 60, 90, and 100. The base image size for this process was 512.




\subsection{Results}  
% \subsubsection{Anatomy Segmentation}
We see quantitative results in Table~\ref{tab:segmentation_results}. We show the performance of selected super-classes and the mean over all 166 classes due to the immense number of classes. We display the complete performance over all classes in Fig.~\ref{fig:bmvc_iou_all_clases}.

In this setting, we find that using pre-trained networks leads to an improvement of up to $\sim14\%$ in mIoU. Additionally, we see that the UNet outperforms the SFPN by approximately $9\%$. However, some classes, such as the heart, lobes, and aorta, see similar performance between the two architectures, while others, such as mediastinal regions, airways, and ribs, show notable differences.
% We see that in the observed setting, we profit from pre-trained networks with a gain from up to $\sim14\,\%$ mIoU. We see a difference in performance based on the architecture as the UNet outperforms the SFPN  by roughly $9\,\%$. While for classes like the heart, lobes, or aorta, these architectures perform similarly, there are noticeable differences for individual mediastinal regions, airways, and ribs.

Overall, we can achieve up to $\sim90\%$ mIoU on certain classes like the spine or heart, but segmentation of lung vessels proves particularly difficult with an IoU of $52\%$. The most significant discrepancy in segmentation quality between the two networks is observed in rib cage segmentation, where the UNet has a gain of $6.1\%$. Figure~\ref{fig:pred_panda} shows qualitative examples of the segmentation results. The vessel tree and tracheal ends towards the bronchi are challenging to segment accurately, while lobe-, intermediastinal-, and bone-related classes appear as expected.
% While we can segment several classes with up to $\sim90\,\%$ mIoU on classes like the spine or heart, the correct segmentation of lung vessels is complicated with an IoU of $52\,\%$. Furthermore, the most significant difference in segmentation quality between the two networks lies in the rib cage segmentation, where the UNet has a gain of $6.1\%$. We observe qualitative examples in Fig.~\ref{fig:pred_panda}. The vessel tree and tracheal ends towards the bronchi pose as difficult, whereas lobe-, intermediastinal-, and bone-related classes appear as expected. 

We demonstrate the usefulness of our proposed dataset for segmenting anatomy in real chest X-Rays by presenting qualitative results on the OpenI dataset in Fig.~\ref{fig:segmentation_results}. 
The segmentation results for various structures, such as the mediastinal classes, sub-diaphragm, lung regions, spine, and ribs, are accurate in both views. However, we observe occasional errors in the prediction of individual ribs, particularly in the overlapping areas with the heart, which the overall brighter region may cause in these areas. Additionally, the predictions of lung vessels appear coarse compared to the annotations, which is expected due to the difficulty in visualizing vessels in chest X-Rays.
Although errors similar to those in projected X-Rays can be seen (e.g., in the lateral rib or diaphragm segmentations), the results are encouraging even without using a domain adaptation method~\cite{toldo2020unsupervised}.
% To show the applicability of our proposed dataset for the anatomy segmentation in real CXR, we display qualitative results on the OpenI dataset in Fig.~\ref{fig:segmentation_results}. 







As we can see, the introduced PAX-Ray dataset enabled glances into the potential of anatomical segmentations in CXR. However, due to the limited size of the dataset, the segmentation of specific sub-classes, such as the individual vertebrae or ribs, becomes difficult to train. Similarly, the human thoracic region consists of more relevant organs, such as the upper abdominal region, than are currently gathered. 

Thus, we propose to extend the PAX-Ray dataset through multiple steps. First, we adapt the translation step between the two modalities to fit the physical underpinnings of Lambert-Beer's law. Secondly, we integrate additional classes by training on other datasets. Previously, we inferred a set of individual models on the entire dataset. This, however, is a massive time sink as depending on the volume spacing  single inference with the nnUNet might take more than 30 minutes. To reduce inference time, we aggregate all classes first on an intermediate full-body CT dataset. Retraining on this merged dataset can translate the knowledge more efficiently to a large set of unannotated thorax CT datasets. We can cut the number of required inferences by a factor of twelve. Lastly, we translate these pseudo-labeled CTs to projected CXR to generate our PAX-Ray++ consisting of more than 14,000 images and 2,000,000 annotated instances. 
We illustrate the entire process in Fig.~\ref{fig:scaling_paxray}.



\subsection{Adjusted Label Accumulation}

For the generation of PAX-Ray, we utilized a combination of a set of learned and non-learned approaches for a diverse set of classes jointly predicted for the RibFrac dataset~\cite{ribfrac2020}. When expanding the dataset, we look at two directions. 
First, increasing the number of observed labels. While the PAX-Ray dataset has many observed classes, it lacks in abdominal organs, heart and lung regions, and several bones. We, thus, gather ten different sources to train networks for subsequent prediction of desired additional classes. 
As labels from these sources can overlap, we first merge the predictions on a single dataset to sort out inconsistencies between annotation schemes and merge similar class labels. Doing so allows us to train a single model on the resulting dataset, significantly reducing inference and postprocessing time when applied to large-scale datasets.
Secondly, we extend the dataset through the amount of considered source CT volumes. Initially, we used a single source dataset of \~440 volumes after filtering, leading to a dataset with less than a thousand images. This amount of images is small compared to several computer vision datasets. Consequently, we collect several large-scale thorax CT datasets to increase the number of projected X-Rays.
Subsequently to these steps, we map these three-dimensional masks to a plane as done with PAX-Ray and filter cases with implausible mask predictions, such as anatomical structures with sizes massively deviating from the mean volume or having multiple connected components despite it being single structure. The masks are then post-processed with standard morphological operations and rescaled to the desired size.



% \input{Chapters/05_learningfrompartialdata/tables/comms/workflow.tex}

\subsubsection{Considered Label Sources}
% \input{Chapters/05_learningfrompartialdata/tables/comms/source_datasets_stats.tex}

We consider datasets focusing on different body systems and available segmentation tools to provide a more leveled label distribution. We use these to train five folds of full resolution nnUNets~\cite{isensee2021nnu} and keep a separate set for validation purposes. For inference, we use an ensemble of all folds with test time augmentation, such as horizontal flipping.
We list the source datasets, their volume information, and the segmentation performance of their resulting networks in Table~\ref{tab:ch5_datasets_overview}. 


The Pediatric dataset~\cite{jordan2022pediatric} contains 287/72 (training/validation) volumes of pediatric patients, with 29 labels spanning the entire body. The segmentation model achieved an IoU of 0.833. The Total Segmentator dataset~\cite{wasserthal2022totalsegmentator} includes 581/146 volumes, with 104 labels for whole body segmentation, including classes such as humerus and the atria of the heart. We achieve an IoU of 0.9251. The SegTHOR dataset~\cite{lambert2020segthor} includes 40/20 volumes, with 5 labels for thoracic organs at risk. We achieve an IoU of 0.9232. The PARSE dataset~\cite{parse} includes 100/30 volumes for pulmonary artery segmentation. On the challenge benchmark, we achieve an IoU of 0.751. The BTCV dataset~\cite{malabdomen} includes 30/20 images, with 14 labels for abdominal segmentation, on which we achieve an IoU of 0.8511. The dataset by Ma et al. ~\cite{ma2021abdomenct} includes 40/10 testing images, with 13 labels for abdominal segmentation. With an IoU of 0.9093. The RibSeg dataset~\cite{yang2021ribseg} includes 420/160 volumes. While the original annotations segment the ribs as a single class along the outskirts of the ribs, we fill the ribs via thresholding and morphological operations and subsequently partition these via connected components into the 12 left and right ribs, with 24 labels for rib segmentation with an IoU of 0.8996. The Verse dataset~\cite{sekuboyina2021verse} includes 112/100 volumes, with 23 labels for vertebrae segmentation. We achieve an IoU of 83.87\%. 
% % \input{Chapters/05_learningfrompartialdata/tables/comms/venndiagram.tex}
We further utilize pre-trained classification models such as the Body Composition Analysis by Koitka~\etal~\cite{koitka2021fully} and the lung lobe segmentation by Hoffmaninger~\etal~\cite{ltrc}.

\subsubsection{Finalizing the Label Structure}

After training the nnUNet ensembles on the individual dataset, we infer the individual models on 560 whole-body volumes of AutoPET~\cite{gatidis2022whole}, a large CT dataset for tumor segmentation covering various body regions. We merge classes of overlapping semantics and discard unnecessary classes or ones of insufficient quality by manual assessment, such as the humerus classes. We further apply postprocessing techniques such as morphological operations and abiding anatomical biases such as maintaining the largest connected component for organs that are supposed to contain a single one. 
% We illustrate the overlap of classes in the Venn-Diagram in Fig.~\ref{fig:venndiagram}.

We then retrain the nnUNet on the resulting dataset. This allows us to generate predictions of the complete label set with just a single model, which is significant as inference and postprocessing for a single ensemble can span up to an hour per volume, making the generation of a large-scale dataset a tall order.
We integrate anatomical regions by modifying several anatomical classes:
\begin{enumerate}
\item The mediastinum stems from the BCA predictions and is split into upper and lower mediastinum along the T4 vertebra.
\item We differentiate the anterior and posterior mediastinum along the heart segmentation boundary.
\item We create the upper and middle lung regions and bases by splitting along the vertical thirds. The apical lung region is defined by the start of the individual clavicles.
\item We define the tracheal bifurcation as starting from 10 slices above the split of the trachea.
\item We maintain the process of the aorta splits and sub-hemidiaphragm from PAX-Ray. 
\end{enumerate}

Furthermore, when projecting the pseudo-labels to a frontal or lateral view, we merge classes to accommodate the characteristics of the view. For example, distinguishing between the left and right breast is impossible in the 
lateral view, whereas this is trivial in the frontal view. On the other hand, the lower mediastinum is better distinguishable in the lateral view, while not in the frontal one. We display the final classes in Fig.~\ref{fig:labelstructure_extendedpaxray}.


\subsubsection{Adjusted CT to X-Ray Projection}\label{sec:matsu}
% \input{Chapters/05_learningfrompartialdata/tables/comms/projectiondifferences.tex}

Our original way of CT back-projection for the generation of the PAX-Ray dataset was focused on visual similarity. However, it was not based on the properties of the attenuation of light. We still split the volume into a body and bone volume for separate processing and subsequent merging, but instead of Eq.~\ref{eq:ch5_init_proj}, we follow Matsubara~\etal~\cite{matsubara2019generation}. This allows us to come closer to a definition of Lambert-Beer's Law of the attenuation of light relating to the material properties it travels through.
However, as CXR generally uses a harder type of radiation, we found that, for the frontal view CXR, further applying histogram equalization~\cite{pizer1987adaptive} leads to more visually pleasing results. We display the differences in translation in Fig.~\ref{fig:difference_in_projection}. We can see that, especially in the basilar lung regions, PAX-Ray++ is darker, while the abdomen is brighter than in our initial work.

% \input{Chapters/05_learningfrompartialdata/tables/comms/label_structure.tex}

\subsubsection{Sources of PAX-Ray++}  
To generate the PAX-Ray++ dataset, we require CT volumes as imaging data. We choose large unlabeled CT datasets focusing on the thoracic region, which is displayed in the bottom part of Table~\ref{tab:ch5_datasets_overview}. 
% \input{Chapters/05_learningfrompartialdata/tables/comms/frontal_images.tex}
% \lipsum[80]

% \input{Chapters/05_learningfrompartialdata/tables/comms/lateral_images.tex}
% \input{Chapters/05_learningfrompartialdata/tables/comms/general_stats.tex}
 The datasets include RSNA PE, RibFrac, LIDC-IDRI, COVID-19-AR, COVID-19-1, and COVID-19-2. 
 The RNSA Pulmonary Embolism dataset, a contrast CT dataset for identifying pulmonary embolisms, is the largest, with more than 7000 volumes with an average axial spacing of 1.25 mm and 237 slices.  
 The RibFrac dataset for detecting rib fractures, which we used for the initial PAX-Ray, consists of 660 volumes with the smallest spacing of 1.13 mm and 359 slices. 
 The LIDC-IDRI dataset was collected to detect pulmonary nodules and consists of 1036 volumes with a spacing of 1.74 and, on average, 237 slices. 
 The COVID-19-AR dataset has, on average, the most slices of 438 and 176 volumes. However, it has a relatively large coronal and sagittal spacing. 
 The COVID-19-1 and -2 datasets contain 215 and 632 volumes but have the smallest amount of slices and the largest axial spacing. 

We infer the nnUNet ensemble trained on the aggregated pseudo-labels on Autopet on these datasets (see Fig.~\ref{fig:scaling_paxray}). We apply the same postprocessing methods as done with the initial predictions on AutoPET and filter volumes with predictions with anatomical deviations, i.e., too few predicted ribs. We then project the image and label files to a frontal and lateral view and resize to a uniform size of $512\times512$ using nearest interpolation for masks and Lanczos~\cite{turkowski1990filters} for images.

 \subsection{Dataset Analysis}
We next investigate the characteristics of PAX-Ray++. 
As each image is generated from a CT volume, the spacing and the slice amount have a noticeable effect on the label and projection quality of the resulting sample. This can be seen in the frontal and lateral qualitative samples in Fig.~\ref{fig:paxray_frontal} and Fig.~\ref{fig:paxray_lateral}. We see the original projections and labels corresponding to the categories \textit{Airways}, \textit{Vascular system}, \textit{Bones} and \textit{abdomen} for the different datasets. The different datasets offer a variety of shades when emulating an X-Ray. The RibFrac and the RSNA PE dataset contain larger abdominal areas, while the remaining datasets focus more on the thoracic region. Due to the lower resolution and slice amount of the COVID-19-1 and -2 datasets, we can note ridges for the segmentations. 

% \input{Chapters/05_learningfrompartialdata/tables/comms/general_stats_small.tex}

We show in Fig.~\ref{fig:paxray_stats} the number of instances per class in the PAX-Ray++ dataset and compare those with the equivalent classes in PAX-Ray. Apart from PAX-Ray++ containing more explicit classes, we can see that overall the instance amount is larger by a magnitude. Furthermore, while all instances occur precisely once per image, the lower ribs and the lower and upper vertebrae do not occur in every image. Similarly, abdominal classes such as the duodenum or stomach are not always visible. Finally, it has to be noted that the breast segmentations are independent of the sex of the patient, as also male participants can show sufficient tissue constellations.  

We compare our PAX-Ray++ dataset against other datasets within and without the CXR domain. These datasets include ChestXDet~\cite{liu2020chestxdet10}, a dataset with mask annotations for pulmonary diseases, CLiP~\cite{tang2021clip}, a dataset with annotations for catheters and lines, our PAX-Ray, as well as the popular natural image datasets PASCAL VOC~\cite{pascal-voc-2007} and MSCOCO~\cite{lin2014microsoft}. 

In Fig.~\ref{fig:dataset_stats_small}a) we compare the number of instances per category against the number of categories. We see that within the domain, PAX-Ray++ provides vastly more different annotations and, in general, provides more annotations
than other datasets within the domain, even comparable to real-world datasets like MS COCO. 

In Fig.~\ref{fig:dataset_stats_small}b) we display the size of each instance annotation relative to the image size. 
The natural image datasets show more instances of taking up more prominent parts of the image, with at least 75\% and 50\% of annotations taking up more than 1\% of the image for PASCAL VOC and MS COCO. On the other hand, CXR datasets mainly consist of smaller annotations. 
We see that nearly all annotations of CLiP are at most 1\% of the image size and at most 0.01\% of annotations taking up 7\%. ChestXDet is more balanced. However, less than 0.1\% of annotations take up more than 20\% of the image. Related to the domain, PAX-Ray++ also consists majorly of more minor instances. However, it also shows instances of up to 70\% of the image.


\subsection{Experimental Setup}
\subsubsection{CT to X-Ray Projection}
Interpreting the quality of the CT to X-Ray backprojection is non-trivial. We seek a correct translation that maintains all physiological features of the CT. Conversely, we want the resulting images to be as close to the X-Ray domain as possible to ease training and improve downstream segmentation tasks. Unfortunately, these properties can not always be maintained due to the differences in the imaging procedure, such as the patient's position since a CT is taken with the patient lying down while in the typical CXR the patient is standing.
To study the quality of the backprojection and the effects of different parts, we utilize the OpenI dataset~\cite{openi} for the computation of the Fr\'echet-Inception Distance~\cite{heusel2017gans}. We calculate the multivariate normal distributions of real ($\mathcal{N}(\mu, \Sigma)$) and 
projected images ($\mathcal{N}(\mu_w, \Sigma_w)$) estimated from Inception v3~\cite{szegedy2016rethinking} features.
\begin{equation}
    \text{FID} = |\mu - \mu_w|_2^2 + tr(\Sigma + \Sigma_w - 2(\Sigma \Sigma_w)^{\frac{1}{2}})
\end{equation}
We evaluate the FID scores on the projection of the RibFrac dataset. We compute the metrics separately for frontal and lateral views. For the extraction of features, all images are resized to $299\times299$.
\subsubsection{Anatomy Segmentation}
We use 30 frontal and lateral images of PAX-Ray++ for the segmentation of anatomical structures as an internal validation set. These images were manually inspected to be visually correct.

To test the real-world applicability of PAX-Ray++ for developing anatomy segmentation models, we prepare a test set of 30 frontal and lateral X-Rays of the PadChest dataset. First, we use our best segmentation model based on the validation performance to generate preliminary anatomical segmentations. Then, we tasked two medical experts to independently examine and correct these densely annotated X-Rays using the annotation tool CVAT~\cite{cvat}. On average, it was reported that even in this simplified annotation process, a single image could take up to 1.5 hours. 

\subsubsection{Implementation Details}
For the projection, we utilize Python 3.10 and packages such as NumPy~\cite{harris2020array} and SciPy~\cite{2020SciPy-NMeth}. All image projections were originally resized to $512\times512$ using Lanczos interpolation.


For our segmentation models, we chose the UNet~\cite{unet} with a ResNet-50~\cite{he2016deep} and ViT-B~\cite{dosovitskiy2020image} backbone. We used pre-trainings on ImageNet~\cite{imagenet} as we did not see a difference in performance to other pre-training methods, i.e., MAE~\cite{he2022masked} on CXRs. As before, we train with binary cross-entropy and employ an additional
binary dice loss. For our base augmentation, we used random resize-and-cropping of range [0.8, 1.2] as augmentation
with an image size of 512 and optimized using AdamW~\cite{loshchilov2017decoupled} with a learning rate of 0.001 for
110 epochs decaying by a factor of 10 at \{60, 90, 100\} epochs. We utilize RandAugment~\cite{cubuk2020randaugment} with $N=9$ and randomized magnitude for heavy augmentation.

\subsection{Results}
\subsubsection{CT to X-Ray Projection}
\noindent\textbf{Effect of Translation Method:}
We first investigate the effect of different translation methods in Fig.~\ref{fig:fid}. Then, we compare the mean intensity projection with Matsubara~\etal~\cite{matsubara2019generation} methods and the other effect of histogram equalization (HE). For the frontal view, we see that the MIP and Matsubara~\etal's method have nearly the same FID to real X-Rays, but when added with HE, Matsubara~\etal shows the best FID with strong visible contrast compared to the originally more faded look.
In the lateral view, HE is not a positive addition, and the original translation by Matsubara~\etal leads to the best results. 
As such, for further projections, we use Matsubara~\etal's method with HE for the frontal case and without for the lateral one. 
% \input{Chapters/05_learningfrompartialdata/tables/wen/notlearned_translation.tex}
% \input{Chapters/05_learningfrompartialdata/tables/wen/ablation_slicethickness.tex}

\noindent\textbf{Effect of Volume Spacing: } Next, we want to investigate the effect that the spacing of a volume can have on the resulting image quality. This is relevant as the dataset we translate can have a variety of axial spacing, as shown in Table~\ref{tab:ch5_datasets_overview}.

We test the spacing 
% \{1,2,3,5\}mm with 
Matsubara~\etal's method. We see that the FID continually increases with the axial spacing. While the difference between 1 and 2 mm is relatively small, further increasing the spacing leads to noticeable differences metrics-wise, while there it is less noticeable from a qualitative perspective. These results might indicate difficulties for networks processing images from 
COVID-19-1/2.

\subsubsection{Projected Anatomy Segmentation}
We use our manually examined validation set to develop the best segmentation model to apply to real-world data and show the results in Fig.~\ref{fig:iou_all_clases}. We first compare the ResNet-50 vs. the ViT-B backbone without using data augmentation. We see that the Resnet-50 outperforms the ViT-B in all classes. Furthermore, we can see minor improvements when adding simple augmentation, which is enhanced when switching to a heavy augmentation setup.  

Generally, we see good performances for standard spinal classes, such as the thoracic vertebrae, while rare vertebrae in the visible thoracic region are more complex. 
It can be noted that classes in the lateral view tend to have better scores than their frontal counterparts, which is also attributed to the fact that frontal classes tend to be finer granular (i.e., left/right split).
Abdominal classes can vary in segmentation quality. For example, while the liver or stomach are typically well-segmented, the duodenum and kidneys are more complex. This, however, might stem from the abdominal region in CXR being relatively bright without strongly noticeable delineations, making it difficult to accurately segment manually.
Heart-related classes show to have near-perfect segmentations with scores above 90\% IoU. 
Individual lung borders are more challenging to identify, leading to scores between 50-60\% IoU.

We show qualitative results in Fig.~\ref{fig:qual_seg_res_proj_frontal} and Fig.~\ref{fig:qual_seg_res_proj_lateral}. Here, we can see classes belonging to the supercategories lungs, vascular systems, bones and abdomen/digestive system. We see that apart from minor deviations at the arterial structure, the segmentations show near to no deviation to the ground truth for both frontal and lateral. 


% \input{Chapters/05_learningfrompartialdata/tables/comms/segmentation_stats.tex}

% \input{Chapters/05_learningfrompartialdata/tables/comms/frontal_segmentations_projections.tex}
% \lipsum[80]
% \input{Chapters/05_learningfrompartialdata/tables/comms/lateral_segmentations_projections.tex}
\subsubsection{X-Ray Anatomy Segmentation}
We show the segmentation performance against medical expert annotations for all classes in Fig.~\ref{fig:iou_all_clases} b). As the task for the human annotators was not to annotate from scratch but to correct wrong pixel-wise predictions, we can see a high agreement for most classes. The most significant disagreements exist for rare bone structures such as L3 and C4, the mediastinal distribution or the breasts. We show the view-wise performance in Fig.~\ref{fig:iou_frontal_lateral}. 
For the frontal classes, high agreement with both annotators can be reached for most classes apart from rare bone structures and the breasts.
In the lateral case, this distinction needs to be clarified. For abdominal and mediastinal classes, annotator 2 aligns more with the model's predictions, while annotator 1 notices some flaws. At the same time, the opposite can be seen for the ribs. 

We display qualitative results in Fig.~\ref{fig:frontal_qual_real} and Fig.~\ref{fig:lateral_qual_real}.
The annotators tend to be content with most annotations. Edits come with extensions of the esophagus, trachea and aorta and corrections of the lower ribs. There is little consensus for some classes, such as the stomach, as can be seen in Fig.~\ref {fig:iou_all_clases} b).
In the lateral view, rib segmentations can become quite hard to interpret. While both annotators disagree with the rib segmentations, they do not agree on how they should look. 
Similarly to the frontal view, tube-like structures like the esophagus are extended as they can appear fractured at times. 

% \input{Chapters/05_learningfrompartialdata/tables/comms/segmentation_stats_sides.tex}

% \input{Chapters/05_learningfrompartialdata/tables/comms/frontal_segmentations_xray.tex}

% \input{Chapters/05_learningfrompartialdata/tables/comms/lateral_segmentations_xray.tex}
\fi
